Quantum references

We present a theory of "quantum references", similar to lenses in classical functional programming, that allow to point to a subsystem of a larger quantum system, and to mutate/measure that part. Mutable classical variables, quantum registers, and wires in quantum circuits are examples of this, but also references to parts of larger quantum datastructures. Quantum references in our setting can also refer to subparts of other references, or combinations of parts from different references, or quantum references seen in a different basis, etc. Our modeling is intended to be well suited for formalization in theorem provers and as a foundation for modeling variables in quantum programs. We study quantum references in greater detail and cover the infinite-dimensional case as well, but also provide a more general treatment not specific to the quantum case. We implemented a large part of our results (including a small quantum Hoare logic and an analysis of quantum teleportation) in the Isabelle/HOL theorem prover.

==> macros.tex <==
\makeatletter

\newcommand{\lemmalabel}[1]{\label{#1}\def\@lemmalabel@current{#1}}
\newcommand{\itlabel}[1]{%
  \protected@write\@auxout{}{\csxdef{@itemlabel@lemma-#1}{\@lemmalabel@current}}%
  \label{#1}
}
\newcommand{\lemmaref}[1]{\ifcsdef{@itemlabel@lemma-#1}{%
    \hyperref[#1]{\autoref*{\csuse{@itemlabel@lemma-#1}}\,(\ref*{#1})}%
  }{\autoref{#1}}}

\newcommand\overlab{a\!b}
\newcommand\overlbc{b\!c}
\newcommand\overlpp{\psi\!\phi}
\newcommand\overlpx{\phi\!\xi}

\newcommand\notanonymous{\ifanonymous \xxx\fi}

\newcommand\footnoterepeat[1]{\textsuperscript{\textnormal{\ref{#1}}}}

\long\def\delaytextsv#1#2{\delaytext{#1}{#2}\fullonly{\usedelayedtext{#1}}}

% \showafter{year}{month}{day}{text} evaluates to {text} starting from year/month/day
\newcommand\showafter[4]{%
  \ifnum\year>#1\relax
    #4% today.year > args.year
  \else
    \ifnum\year=#1\relax
    % today.year = args.year
      \ifnum\month>#2\relax
      % today.month > args.month
        #4%
      \else
        \ifnum\month=#2\relax
        % today.month = args.month
          \ifnum\day>#3\relax
          % today.day >= args.day
            #4%
          \else
            \ch@removeduplicatespace
          \fi
        \else
          \ch@removeduplicatespace
        \fi
      \fi
    \else
      \ch@removeduplicatespace
    \fi
  \fi}


\newcommand\txtrel[1]{\stackrel{\hskip-1in\text{\tiny#1}\hskip-1in}}
\newcommand{\eqrefrel}[1]{\txtrel{\eqref{#1}}}
\newcommand\starrel{\txtrel{$(*)$}}
\newcommand\starstarrel{\txtrel{$(**)$}}
\newcommand\tristarrel{\txtrel{$\scriptscriptstyle (\!*\!*\!*\!)$}}
\newcommand\fourstarrel{\txtrel{$\scriptscriptstyle (\!*\!*\!*\!*\!)$}}
\newcommand\fivestarrel{\txtrel{$\scriptscriptstyle (\!*\!*\!*\!*\!*\!)$}}
\newcommand\selfbutter[1]{\butter{#1}{#1}}
\newcommand\butter[2]{\ket{#1}\bra{#2}}
\newcommand\pagelabel[1]{\phantomsection\label{#1}}

\newcommand\calD{\mathcal D}

\def\parenthesis@resizecommand@gobblemaybe#1{\ifx#1.\else#1\fi}
%\def\parenthesis@resizecommand@gobblemaybe#1{#1}
\def\parenthesis@resizecommand@open{\parenthesis@resizecommand@gobblemaybe}
\def\parenthesis@resizecommand@close{\parenthesis@resizecommand@gobblemaybe}
\def\parenthesis@#1#2#3#4#5{%
  \global\def\parenthesis@resizecommand@open{\parenthesis@resizecommand@gobblemaybe}%
  \global\def\parenthesis@resizecommand@close{\parenthesis@resizecommand@gobblemaybe}%
  #1#3%
  {#5}%
  #2#4%
}
\DeclareRobustCommand\parenthesis[3]{%
  \expandafter\expandafter\expandafter
  \parenthesis@\expandafter\expandafter\expandafter{\expandafter\parenthesis@resizecommand@open\expandafter}\expandafter{\parenthesis@resizecommand@close}{#1}{#2}{#3}}


% #1=bigl #2=bigr #3=( #4=txt #5=) #6=txt #7=( #8=txt #9=)
\def\double@parenthesis@#1#2#3#4#5#6#7#8#9{%
  \global\def\parenthesis@resizecommand@open{\parenthesis@resizecommand@gobblemaybe}%
  \global\def\parenthesis@resizecommand@close{\parenthesis@resizecommand@gobblemaybe}%
  #1#3{#4}#2#5%
  {#6}%
  #1#7{#8}#2#9%
}

\DeclareRobustCommand\doubleParenthesis[7]{%
  \expandafter\expandafter\expandafter
  \double@parenthesis@\expandafter\expandafter\expandafter{\expandafter\parenthesis@resizecommand@open\expandafter}\expandafter{\parenthesis@resizecommand@close}{#1}{#2}{#3}{#4}{#5}{#6}{#7}}


\DeclareRobustCommand\resize@next@paren[2]{%
  \gdef\parenthesis@resizecommand@open{#1}%
  \gdef\parenthesis@resizecommand@close{#2}%
}

\newcommand\paren{\parenthesis()}
\newcommand\braces{\parenthesis\{\}}
\newcommand\bracket{\parenthesis[]}

\newcommand\pb{\resize@next@paren\bigl\bigr}
\newcommand\pbb{\resize@next@paren\biggl\biggr}
\newcommand\plr{\resize@next@paren\left\right}
\newcommand\pB{\resize@next@paren\Bigl\Bigr}
\newcommand\pBb{\resize@next@paren\biggl\biggr}

\newcommand\bit{\braces{0,1}}
\newcommand\bits[1]{\bit^{#1}}
\newcommand\frakP{\mathfrak P}
\newcommand\cupdot{\mathbin{\mathaccent\cdot\cup}}

\declare{macro=\assign, argspec=[2], code={#1\leftarrow #2}, nopage=true,
  placeholder={\assign xe},
  description={Assign (the result of evaluating) $e$ to $x$}}

\newcommand\qapplyOLD[2]{\qapply{#2}{#1}}
\declare{macro=\qapply, argspec=[2], code={\mathbf{apply}\ #1\ \mathbf{to}\ #2},
  placeholder={\qapply XU},
  description={Apply the unitary $U$ to quantum reference $X$}}

\declare{macro=\skipprog, code=\mathbf{skip},
  description={Empty program (a.k.a.~skip)}}

\declare{macro=\qif, argspec=[4], code={\mathbf{if}\ \paren{{#1}={#2}}\ {#3}\ \mathbf{else}\ {#4}},
  placeholder={\qif FxPQ},
  description={Run $P$ if $F$ contains $\ket x$, otherwise $Q$}}


\declare{macro=\chain, argspec=[2], code={#1.#2},
  placeholder=\chain FG,
  description={Reference $G$ inside reference $F$ (chaining)}}

\declare{macro=\spair, argspec=[2], code={#1#2},
  placeholder=\spair FG,
  description={Pair of references $F$ and $G$ (right-associative), same as $\pair FG$}}
\newcommand\spairFFF[3]{#1#2#3}
\declare{macro=\pair, argspec=[2], code={\paren{#1,#2}},
  placeholder=\pair FG,
  description={Pair of references $F$ and $G$ (right-associative), same as $\spair FG$}}
\newcommand\pairs[2]{\paren{#1,\dots,#2}}
\newcommand\pairFFF[3]{\paren{#1,#2,#3}}
\newcommand\pairFdFF[3]{\paren{#1,\dots,#2,#3}}
\newcommand\pairFdFFF[4]{\paren{#1,\dots,#2,#3,#4}}
\newcommand\pairFdFFdF[4]{\paren{#1,\dots,#2,#3,\dots,#4}}

\declare{macro=\basistrafo, argspec=[2], code={#1\cdot#2},
  placeholder=\basistrafo UF,
  description={Basis transformation of register $F$ using unitary $U$}}

\declare{macro=\denot, argspec=[1], code={\llbracket#1\rrbracket},
  placeholder=\denot x,
  description={Denotational semantics of (program/variables/\dots) $x$}}

\declare{macro=\ket, argspec=[1], code={\parenthesis\lvert\rangle{#1}}, nopage=true,
  placeholder=\ket x,
  description={Computational basis state}}

\declare{macro=\bra, argspec=[1], code={\parenthesis\langle\rvert{#1}}, nopage=true,
  placeholder=\bra x,
  description={Adjoint of computational basis state}}

\declare{macro=\calH, code=\mathcal H, nopage=true,
  description={A Hilbert space}}
\newcommand\calK{\mathcal K}

\declare{macro=\CNOT, code=\mathsf{CNOT}, nopage=true,
  description={Controlled-NOT gate/matrix}}

\declare{macro=\hada, code=\mathsf H,
  description={Hadamard matrix}}

\declare{macro=\pauliX, code=\sigma_x,
  description={Pauli $X$-matrix}}

\declare{macro=\pauliZ, code=\sigma_z,
  description={Pauli $Z$-matrix}}

\declare{macro=\setC, code=\mathbb C, nopage=true,
  description={Complex numbers}}
\declare{macro=\setR, code=\mathbb R, nopage=true,
  description={Real numbers}}
\declare{macro=\setN, code=\mathbb N, nopage=true,
  description={Natural numbers}}
\declare{macro=\setZ, code=\mathbb Z, nopage=true,
  description={Integers}}

\declare{macro=\adj, argspec=[1], code={#1^\dagger}, nopage=true,
  placeholder=\adj A,
  description={Adjoint / conjugate transpose}}

\declare{macro=\letin, argspec=[3], code={\mathsf{let}\ #1:=#2\ \mathsf{in}\ #3}, nopage=true,
  placeholder=\letin xyz,
  description={Evaluate $z$ with $x:=y$. Same as $(\lambda x.z)y$.}}

\declare{macro=\calR, code=\mathcal R, nopage=true,
  description={A reference category}}

\declare{macro=\Fst, code=\mathsf{Fst},
  description={Reference: first part of a bipartite system}}

\declare{macro=\Snd, code=\mathsf{Snd},
  description={Reference: first part of a bipartite system}}

\declare{macro=\id, code=\mathit{id}, nopage=true,
  description={Identity}}

\declare{macro=\Lquantumfin, code=\calR_\mathit{quantum}^\mathit{fin},
  description={Reference category for the quantum setting, finite-dimensional}}

\declare{macro=\Lquantum, code=\calR_\mathit{quantum},
  description={Reference category for the quantum setting, infinite-dimensional}}

\declare{macro=\Lclassical, code=\calR_\mathit{classical},
  description={Reference category for the classical setting}}

\declare{macro=\sandwich, argspec=[1], code=\mathsf{Sd}_{#1},
  placeholder=\sandwich U,
  description={Sandwich, $a\mapsto Ua\adj U$}}

\declare{macro=\im, code=\operatorname{im}, nopage=true,
  placeholder=\im a,
  description={Image of $a$}}

\declare{macro=\hoare, argspec=[3], code={\doubleParenthesis\{{#1}\}{#2}\{{#3}\}},
  placeholder=\hoare FPG,
  description={Quantum Hoare judgment}}

\declare{macro=\Span, code=\operatorname{span}, nopage=true,
  placeholder=\Span S,
  description={Linear span of set $S$}}

\declare{macro=\quanteq, code={=_q},
  placeholder={F\quanteq \psi},
  description={Intuitively: reference $F$ is in state $\psi$}}

\declare{macro=\teleport, code=\mathsf{Teleport},
  placeholder=\teleport,
  description={Teleportation program}}

\declare{macro=\bell, code=\beta_{00},
  description={EPR pair / Bell state $\frac1{\sqrt2}\ket{00} + \frac1{\sqrt2}\ket{11}$}}

\declare{macro=\CBL, code={\Rightarrow_\mathit{CL}},
  placeholder=\alpha \CBL \beta,
  description={Short for Isabelle/HOL type $(\alpha,\beta)$ \texttt{cblinfun}}}

\declare{macro=\tr, code=\operatorname{tr}, nopage=true,
  placeholder=\tr A,
  description={Trace of operator/matrix $A$}}

\declare{macro=\norm, argspec=[1], code={\parenthesis\lVert\rVert{#1}}, nopage=true,
  placeholder=\norm A,
  description={Norm of $A$ (either Hilbert space norm, or operator norm)}}

\declare{macro=\trnorm, argspec=[1], code=\norm{#1}_{\tr},
  placeholder=\trnorm A,
  description={Trace norm of $A$}}

\declare{macro=\abs, argspec=[1], code={\parenthesis\lvert\rvert{#1}}, nopage=true,
  placeholder=\abs x,
  description={Absolute value of $x$}}

\declare{macro=\comm, argspec=[1], code=#1',
  placeholder=\comm{\mathbf A},
  description={Commutant of von Neumann algebra $\mathbf A$}}

\declare{macro=\idmult, code=\setC1,
  description={Set of multiples of the identity operator}}

\declare{macro=\induction, argspec=[2], code=(#1)_{#2},
  placeholder=\induction x{e'},
  description={Induction map}}

\newcommand\XAB{\pb\pair{\spair XA}B}
\newcommand\PhiOne{\chain\Phi\Fst}
\newcommand\PhiTwo{\chain\Phi\Snd}
\newcommand\XPhi{\spair X\Phi}
\newcommand\XPhiOne{\pair X\PhiOne}
\newcommand\XPhiTwo{\pair X\PhiTwo}
\newcommand\PhiTwoAB{\pb\pair{\pair\PhiTwo A}B}
\newcommand\pre{\mathord\spadesuit}
\newcommand\XZ{\pauliZ^b\pauliX^a}
\newcommand\XZadj{\pauliX^a\pauliZ^b}

\declare{macro=\rtensor, code=\otimes_{\mathbf r},
  placeholder=F\rtensor G,
  description={Tensor product of references (right-associative)}}

\declare{macro=\atensor, code=\otimes_{\mathrm{alg}},
  placeholder=\mathbf A\atensor\mathbf B,
  description={Algebraic tensor product}}

\declare{macro=\stensor, code=\otimes_{\mathrm{sp}},
  placeholder=\mathbf A\stensor\mathbf B,
  description={Spatial tensor product}}

\declare{macro=\tensor, code=\otimes,
  description={Tensor product of update monoids, Hilbert spaces, or von Neumann algebras (right-associative)}}

\declare{macro=\bounded, code=B,
  placeholder=\bounded(\calH),
  description={Bounded operators on $\calH$. We abbreviate $\bounded(\calH_A),\bounded(\calH_B),\dots$ as $\mathbf A,\mathbf B,\dots$}}

\declare{macro=\tracecl, code=T,
  placeholder=\tracecl(\calH),
  description={Trace-class operators on $\calH$}}

\declare{macro=\calE, code=\mathcal E, nopage=true,
  placeholder={\calE,\calF,\calG},
  description={Usually denotes a quantum (sub)channel}}
\newcommand\calF{\mathcal F}
\newcommand\calG{\mathcal G}

\declare{macro=\conj, argspec=[1], code={\overline{#1}},
  placeholder=\conj x,
  description={Complex conjugate of $x$}}

\declare{macro=\Uswap, code=U_\sigma,
  description={Two-qubit swap unitary}}

\declare{macro=\swap, code=\sigma,
  description={Swap (reference)}}

\declare{macro=\assoc, code=\alpha,
  description={Associator (reference)}}

\declare{macro=\assocp, code=\alpha',
  description={Associator (reference)}}

\newcommand\sectionToToc{%
  \let\OLDsection\section
  \def\section*##1{%
    \OLDsection*{##1}%
    \addcontentsline{toc}{section}{##1}%
  }%
}

\declare{macro=\partialto, code=\rightharpoonup,
  placeholder={A\partialto B},
  description={Partial functions from $A$ to $B$}}

\declare{macro=\compl, argspec=[1], code={#1^\complement},
  placeholder=\compl F,
  description={Complement of reference $F$}}

\declare{macro=\unitreg, argspec=[1], code={U_{#1}},
  placeholder=\unitreg{\mathbf A},
  description={Unit reference with codomain $\mathbf A$}}

\declare{macro=\regsubspace, argspec=[2], code={#1\paren{#2}},
  placeholder=\regsubspace FS,
  description={Lifting a closed subspace $S$ through a reference $F$}}

\declare{macro=\regchannel, argspec=[2], code={#1\paren{#2}},
  placeholder=\regchannel F\calE,
  description={Lifting a quantum channel $\calE$ through a reference $F$}}

\declare{macro=\regmeas, argspec=[2], code={#1\paren{#2}},
  placeholder=\regchannel FM,
  description={Lifting a measurement $M$ through a reference $F$}}

\declare{macro=\unicornX, code={\!\includegraphics[height=2.2ex]{Unicorn-Silhouette-3.pdf}},
  description={Unicorn\symbolindexmarkonly\unicornX}}

\declare{macro=\trin, argspec=[1], code={\tr_{\downarrow#1}},
  placeholder=\trin F,
  description={Partial trace (tracing in $F$)}}

\declare{macro=\trinFst, code={\trin\Fst},
  description={Partial trace (special case for $\Fst$)}}

\declare{macro=\pureeta, argspec=[1], code={\eta_{#1}},
  placeholder=\pureeta{\mathbf A},
  description={Auxiliary vector in $\calH_A$ for pure state lifting}}
\newcommand\pureetabutt[1]{\pureeta{#1}\adj{\pureeta{#1}}}

\declare{macro=\purexi, argspec=[1], code={\xi_{#1}},
  placeholder=\purexi b,
  description={Auxiliary vector for pure state lifting}}

\declare{macro=\ptensor, code={\otimes_{\mathfrak p}},
  placeholder=F(\psi)\ptensor G(\phi)\ptensor\dots,
  description={Lifting of pure states $\psi,\phi,\dots$ through references $F,G,\dots$}}

\declare{macro=\mtensor, code={\otimes_{\mathfrak m}},
  placeholder=F(\rho)\mtensor G(\sigma)\mtensor\dots,
  description={Lifting of mixed states $\rho,\sigma,\dots$ through references $F,G,\dots$}}

\declare{macro=\ortho, argspec=[1], code=#1^\bot,
  placeholder=\ortho S,
  description={Orthogonal complement of subspace $S$}}

\declare{macro=\Sem, code=\mathbf{Sem},
  placeholder=\Sem_T,
  description={Program semantics for memory of type $T$}}

\declare{macro=\proccall, argspec=[2], code=\mathbf{call}\ #1\paren{#2},
  placeholder=\proccall pX,
  description={Procedure call}}

\declare{macro=\procdef, argspec=[3], code={\mathbf{proc}\ #1(\prm : #2)\ \braces{#3}},
  placeholder=\procdef pTP,
  description={Procedure declaration}}


\declare{macro=\prm, code=\mathbf{prm},
  description={Placeholder for procedure parameters}}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "references"
%%% End:

